EMO-LLaMA: Enhancing Facial Emotion Understanding with Instruction Tuning

Facial expression recognition (FER) is an important research topic in emotional artificial intelligence. In recent decades, researchers have made remarkable progress. However, current FER paradigms face challenges in generalization, lack semantic information aligned with natural language, and struggle to process both images and videos within a unified framework, making their application in multimodal emotion understanding and human-computer interaction difficult. Multimodal Large Language Models (MLLMs) have recently achieved success, offering advantages in addressing these issues and potentially overcoming the limitations of current FER paradigms. However, directly applying pre-trained MLLMs to FER still faces several challenges. Our zero-shot evaluations of existing open-source MLLMs on FER indicate a significant performance gap compared to GPT-4V and current supervised state-of-the-art (SOTA) methods. In this paper, we aim to enhance MLLMs' capabilities in understanding facial expressions. We first generate instruction data for five FER datasets with Gemini. We then propose a novel MLLM, named EMO-LLaMA, which incorporates facial priors from a pretrained facial analysis network to enhance human facial information. Specifically, we design a Face Info Mining module to extract both global and local facial information. Additionally, we utilize a handcrafted prompt to introduce age-gender-race attributes, considering the emotional differences across different human groups. Extensive experiments show that EMO-LLaMA achieves SOTA-comparable or competitive results across both static and dynamic FER datasets. The instruction dataset and code are available at https://github.com/xxtars/EMO-LLaMA.

==> Euqation/addffn.tex <==
\begin{equation}
\tilde{\textbf{X}}^{V}_t = \operatorname{FFN}(\textbf{X}^{AU,\,global}_t + \textbf{X}^{AU,\,local}_t).
\end{equation}

==> Euqation/au_center.tex <==
\begin{equation}
\begin{aligned}
AU^{1,\,left}_x & = L^{22}_x, \\
AU^{1,\,left}_y & = L^{22}_y-\frac{\xi'}{2},
\label{e:aucenter}
\end{aligned}
\end{equation}

==> Euqation/corrected_au_center.tex <==
\begin{equation}
\begin{aligned}
AU^{1,\,left}_x & = L^{22}_x - \frac{\xi \times \cos(\text{Pitch}) \times \sin(\theta^v)}{2}, \\
AU^{1,\,left}_y & = L^{22}_y-\frac{\xi \times \cos(\text{Pitch}) \times \cos(\theta^v)}{2}.
\label{e:c_aucenter}
\end{aligned}
\end{equation}

==> Euqation/face_sattn.tex <==
\begin{equation}
\hat{\textbf{X}}^{V}_t = \operatorname{SAttn}(\textbf{X}^V_t),
\end{equation}

==> Euqation/faceinfomini.tex <==
\begin{equation}
\begin{aligned}
\tilde{\textbf{X}}^V_t = &\operatorname{FFN}(\operatorname{GFAttn}(\operatorname{SAttn}(\textbf{X}^V_t), \textbf{X}^F_t)) \\
& +\operatorname{LFAttn}(\operatorname{SAttn}(\textbf{X}^V_t), \textbf{X}^F_t, \textbf{X}^L_t)).
\end{aligned}
\end{equation}

==> Euqation/gfattn.tex <==
\begin{equation}
\begin{aligned} 
\textbf{X}^{V,\,global}_t & = \operatorname{GFAttn}(\hat{\textbf{X}}^V_t, \textbf{X}^F_t), \\
& = \operatorname{XAttn}(\hat{\textbf{X}}^V_t, \textbf{X}^F_t) + \hat{\textbf{X}}^V_t,
\end{aligned}
\end{equation}

==> Euqation/lfattn.tex <==
\begin{equation}
\begin{aligned} 
\textbf{X}^{V,\,local}_t & = \operatorname{LFAttn}(\hat{\textbf{X}}^V_t, \textbf{X}^F_t, \textbf{X}^L_t), \\
& = \operatorname{XAttn}(\hat{\textbf{X}}^V_t, \textbf{X}^{AU,\,local}_t) + \hat{\textbf{X}}^V_t, \\
\textbf{X}^{AU,\,local}_t & = \operatorname{AUCL}(\textbf{X}^{AU,\,ROI}_t)),
\end{aligned}
\end{equation}

==> Euqation/scale.tex <==
\begin{equation}
\begin{aligned}
\xi' & = \operatorname{D}(L^{41}, L^{43}), \\
\xi & = \frac{\xi'}{\cos(\text{Yaw})}, \\
\operatorname{D}(L^{i}, L^{j}) & = \sqrt{(L^{j}_x - L^{i}_x)^2 + (L^{j}_y - L^{i}_y)^2},
\label{e:scale}
\end{aligned}
\end{equation}

==> Euqation/vertical.tex <==
\begin{equation}
\begin{aligned}
& L^{left\_eye} = \operatorname{Centroid}(L^{37}, L^{38}, L^{39}, L^{40}, L^{41}, L^{42}), \\
& L^{right\_eye} = \operatorname{Centroid}(L^{43}, L^{44}, L^{45}, L^{46}, L^{47}, L^{48}), \\
& L^{center\_eye} = \operatorname{Centroid}(L^{left\_eye}, L^{right\_eye}), \\
& L^{center\_mouth} = \operatorname{Centroid}(L^{49}, L^{50}, L^{51}, L^{52}, L^{53}, L^{54}, \\
& L^{55}, L^{56}, L^{57}, L^{58}, L^{59}, L^{60}), \\
& \theta^v = \arctan(\frac{|L^{center\_mouth}_x - L^{center\_eye}_x|}{|L^{center\_mouth}_y - L^{center\_eye}_y|}), \\
& \operatorname{Centroid}(\{L^i\}_{i=1}^{n}) = \frac{1}{n} \sum_{i=1}^{n} L^i.
\label{e:vertival}
\end{aligned}
\end{equation}

==> Table/crossmodality_image.tex <==
\begin{table}
  \caption{Evaluation of EMO-LLaMA on the image modality trained with video modality data. \textit{general} means pre-training on general purpose images or videos, \textit{video} refers to pre-training on FER-related videos.}
  \label{tab:crossmodality_image}
  \centering
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}}
    \toprule
    \multirow{2}{*}{Methods} & \multirow{2}{*}{Training Modality} & AffectNet & RAF-DB & FERPlus \\ 
    & & Acc & Acc & Acc \\
    \midrule
    \multicolumn{5}{c}{\textit{Zero-shot of MLLMs}} \\
    LLaMA-VID~\cite{li2023llama} & \textit{general} & 32.96 & 57.66 & 49.45 \\
    GPT-4V~\cite{achiam2023gpt,lian2023gpt} & - & \textbf{42.77} & \textbf{75.81} & \textbf{64.25} \\
    \midrule
    EMO-LLaMA (Ours) & \textit{video} & 38.31 & 71.32 & 59.08 \\
    \bottomrule
  \end{tabular*}
\end{table}

==> Table/face_info_mini.tex <==
\begin{wrapfigure}{t}{0.3\textwidth}
    \centering
    \vspace{-1em}
    \caption{Ablation study of Face Info Mining}
    \vspace{-0.5em}
    \label{tab:faceinfomini}
      \begin{tabular*}{0.3\textwidth}{@{\extracolsep{\fill}}l@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}}
        \toprule
        \multirow{2}{*}{Strategy} & \multicolumn{2}{c}{MAFW} \\ \cmidrule(rl){2-3}
        & UAR & WAR  \\ 
        \midrule
         Pool \& Concat&  &  \\
         Face Info Mining &  & \\
        \bottomrule
      \end{tabular*}
    \vspace{-1.5em}
\end{wrapfigure}

==> Table/facialprior.tex <==
\begin{table}
  \caption{Ablation study on facial priors.}
  \label{tab:facial_prior}
  \centering
  \footnotesize
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}}
    \toprule
    \multirow{2}{*}{Facial Embedding} & \multirow{2}{*}{Landmark} & \multirow{2}{*}{ARG} & \multicolumn{2}{c}{MAFW} \\ \cmidrule(rl){4-5}
    & & & UAR & WAR  \\ 
    \midrule
    & & & &  \\
    \checkmark & & & &  \\
    \checkmark & \checkmark & & &  \\
    \checkmark & \checkmark & \checkmark & &  \\
    \bottomrule
  \end{tabular*}
\end{table}

==> Table/instruction_static.tex <==
\begin{table}[t]
    \centering
    \captionof{table}{Statistics of selected FER datasets.}
      \label{tab:statistics}
      \small
      \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}}
        \toprule
        \multirow{2}{*}{Datasets} & \multirow{2}{*}{Annotation} & Data & Instruction &  Long-tail \\
        & & Number & Number & Ratio \\
        \midrule
        FERPlus & 8 expressions & 29k & - & 61 \\
        RAF-DB & 7 expressions & 12k & 12k & 17 \\
        AffectNet & 8 expressions & 288k & 283k & 36 \\
        DFEW & 7 expressions & 9k & 7k & 18 \\
        FERV39K & 7 expressions & 31k & 30k & 5 \\
        MAFW & 11 expressions \& short text & 7k & 7k & 8 \\
        
        \bottomrule
      \end{tabular*}
\end{table}

==> Table/mafw_map.tex <==
\begin{table}
  \caption{Zeroshot on MAFW set1 of MLLMs}
  \label{MAFW_map}
  \centering
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}}
    \toprule
     \multirow{2}{*}{Methods} & \multicolumn{11}{c}{Accuracy of each expression (\%)} & \multicolumn{4}{c}{Metric} \\
    \cmidrule(rl){2-12} \cmidrule(rl){13-16}
    & AN & DI & FE & HA & NE & SA & SU & CO & AX & HL & DS & UAR & WAR & UF1 & WF1 \\
    \midrule
    \midrule
    Chat-UniVi\textsuperscript{v} & 3.24 & 7.81 & 0.80 & 83.94 & 0.00 & 70.07 & 13.95 & 54.17 & 3.80 & 0.00 & 5.41 & \underline{22.11} & \underline{27.19} & \underline{15.52} & \underline{21.23} \\
    Chat-UniVi\textsuperscript{v+t} & 20.14 & 21.09 & 0.80 & 40.96 & 0.00 & 87.07 & 25.58 & 52.08 & 9.78 & 0.00 & 16.22 & 24.89 & 29.69 & 19.83 & 26.67 \\
    \midrule
    Video-ChatGPT\textsuperscript{v} & 50.72 & 0.78 & 0.00 & 6.83 & 14.04 & 32.31 & 51.16 & 6.25 & 0.00 & 0.00 & 0.00 & 14.74 & 21.70 & 11.79 & 17.49 \\
    Video-ChatGPT\textsuperscript{v+t} & 34.17 & 16.41 & 0.80 & 8.84 & 0.44 & 24.83 & 62.33 & 2.08 & 0.00 & 0.00 & 0.00 & 13.63 & 18.92 & 10.63 & 15.11 \\
    \midrule
    Video-LLaMA\textsuperscript{v} & 2.52 & 1.56 & 2.42 & 85.14 & 44.30 & 80.61 & 3.72 & 0.00 & 0.00 & 0.00 & 0.00 & 20.02 & 31.00 & 13.27 & 19.91 \\
    Video-LLaMA\textsuperscript{v+a} & 6.12 & 0.78 & 0.80 & 79.92 & 29.39 & 88.44 & 3.26 & 0.00 & 0.00 & 0.00 & 0.00 & 18.97 & 30.02 & 13.03 & 19.90 \\
    Video-LLaMA\textsuperscript{v+t} & 13.31 & 8.59 & 16.80 & 73.90 & 39.47 & 95.92 & 17.67 & 4.17 & 1.09 & 0.00 & 2.70 & 24.87 & 36.32 & 22.49 & 30.35 \\
    Video-LLaMA\textsuperscript{v+a+t} & 25.54 & 10.16 & 11.20 & 63.86 & 27.19 & 98.98 & 16.74 & 2.08 & 1.09 & 0.00 & 2.70 & 23.59 & 35.35 & 21.76 & 29.91 \\
    \midrule
    OneLLM\textsuperscript{v} & 0.36 & 9.38 & 18.40 & 32.13 & 10.09 & 71.43 & 10.70 & 81.25 & 0.00 & 1.89 & 2.70 & 21.67 & 22.46 & 16.82 & 21.47 \\
    OneLLM\textsuperscript{v+t} & 0.36 & 21.88 & 24.80 & 25.70 & 1.75 & 63.61 & 6.05 & 95.83 & 0.00 & 0.00 & 0.00 & 21.82 & 20.34 & 16.06 & 20.48 \\
    \midrule
    LLaMA-VID\textsuperscript{v} & 8.99 & 67.97 & 3.20 & 36.55 & 0.44 & 63.61 & 8.37 & 22.92 & 0.54 & 0.00 & 0.00 & 19.26 & 23.11 & 14.98 & 20.76 \\
    LLaMA-VID\textsuperscript{v+t} & 12.23 & 80.47 & 6.40 & 28.92 & 1.32 & 64.97 & 26.51 & 8.33 & 0.54 & 0.00 & 0.00 & 20.88 & 25.72 & 17.18 & 23.88 \\
    LLaMA-VID\textsuperscript{v, mixv2e3} & 42.81 & 11.72 & 20.80 & 79.12 & 78.51 & 47.62 & 43.28 & 0.00 & 23.37 & 0.00 & 0.00 & 31.56 & 44.15 & 30.58 & 41.98 \\
    LLaMA-VID\textsuperscript{v, mixv3e3} & 42.09 & 18.75 & 27.20 & 79.52 & 72.81 & 57.14 & 42.33 & 2.08 & 19.57 & 0.00 & 0.00 & \textbf{32.86} & \textbf{45.41} & \textbf{32.13} & \textbf{43.67} \\
    LLaMA-VID\textsuperscript{v+t, mixv2e3} & 57.91 & 29.69 & 28.00 & 77.11 & 72.81 & 61.90 & 61.40 & 0.00 & 25.54 & 0.00 & 0.00 & \textbf{37.67} & \textbf{51.82} & \textbf{36.50} & \textbf{49.66} \\
    \midrule
    \midrule
    \bottomrule
  \end{tabular*}
  {\raggedright \textsuperscript{v} represents video modality; \textsuperscript{t} represents text modality; \textsuperscript{a} represents audio modality; \par}
\end{table}


==> Table/microfer.tex <==
\begin{wrapfigure}{t}{0.3\textwidth}
    \centering
    \vspace{-1em}
    \caption{Zero-shot evaluation of EMO-LLaMA on micro-expression recognition.}
    \vspace{-0.5em}
    \label{tab:microfer}
      \begin{tabular*}{0.3\textwidth}{@{\extracolsep{\fill}}l@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}}
        \toprule
        \multirow{2}{*}{Methods} & CASME \uppercase\expandafter{\romannumeral2} \\ \cmidrule(rl){2-2}
        & Acc  \\ 
        \midrule
        \multicolumn{2}{c}{\textit{Zero-shot of MLLMs}} \\
         LLaMA-VID~\cite{li2023llama} & 12.89 \\
         GPT-4V~\cite{achiam2023gpt,lian2023gpt} & 14.64 \\
         \midrule
         EMO-LLaMA & 25.00 \\
        \bottomrule
      \end{tabular*}
    \vspace{-1.5em}
\end{wrapfigure}

==> Table/zeroshot.tex <==
\begin{table*}
  \caption{Zero-shot performance comparison on facial expression recognition.}
  \label{tab:zeroshot}
  \centering
  \small
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}c@{\extracolsep{\fill}}}
    \toprule
    \multirow{2}{*}{Methods} & \multicolumn{1}{c}{AffectNet} & \multicolumn{1}{c}{RAF-DB} & \multicolumn{1}{c}{FERPlus} & \multicolumn{2}{c}{DFEW} & \multicolumn{2}{c}{FERV39K} & \multicolumn{2}{c}{MAFW} \\ 
    \cmidrule(rl){2-2} \cmidrule(rl){3-3} \cmidrule(rl){4-4} \cmidrule(rl){5-6} \cmidrule(rl){7-8} \cmidrule(rl){9-10}
    & Acc & Acc & Acc & UAR & WAR & UAR & WAR & UAR & WAR \\
    \midrule
    \multicolumn{10}{c}{\textit{Zero-shot of Contrastive Learning Methods}} \\
    CLIP~\cite{radford2021learning, foteinopoulou2023emoclip} & - & - & - & 19.86 & 10.60 & 20.99 & 17.10 & 20.04 & 21.00 \\
    EmoCLIP~\cite{foteinopoulou2023emoclip} & - & - & - & 36.76 & 46.27 & 26.73 & 35.30 & 25.86 & 33.49 \\
    \midrule
    \multicolumn{10}{c}{\textit{Zero-shot of existing MLLMs}} \\
    Video-ChatGPT~\cite{maaz2023video} & 29.53 & 15.68 & 43.62 & 25.87 & 33.19 & 23.22 & 24.32 & 14.74 & 21.70 \\
    Video-LLaMA~\cite{zhang2023video} & 26.23 & 54.37 & 52.46 & 24.86 & 35.03 & 17.81 & 22.71 & 20.02 & \textbf{31.00} \\
    Chat-UniVi~\cite{jin2023chat} & 27.90 & 59.16 & 44.36 & 32.93 & 37.29 & 21.76 & 25.68 & \textbf{22.11} & 27.19 \\
    LLaMA-VID~\cite{li2023llama} & 32.96 & 57.66 & 49.45 & 33.01 & 38.36 & \textbf{25.97} & 30.55 & 19.33 & 23.11 \\
    OneLLM~\cite{han2023onellm}  & 31.71 & 38.43 & 42.63 & 31.58 & 30.88 & 24.22 & 30.65 & 21.67 & 22.46 \\
    GPT-4V~\cite{achiam2023gpt,lian2023gpt} & \textbf{42.77} & \textbf{75.81} & \textbf{64.25} & \textbf{36.96} & \textbf{43.80} & 24.92 & \textbf{34.19} & - & - \\
    \bottomrule
  \end{tabular*}
\end{table*}

